Effective and Privacy preserving Tabular Data Synthesizing

While data sharing is crucial for knowledge development, privacy concerns and strict regulation (e.g., European General Data Protection Regulation (GDPR)) unfortunately limits its full effectiveness. Synthetic tabular data emerges as an alternative to enable data sharing while fulfilling regulatory and privacy constraints. The state-of-the-art tabular data synthesizers draw methodologies from Generative Adversarial Networks (GAN). In this thesis, we develop CTAB-GAN, a novel conditional table GAN architecture that can effectively model diverse data types with complex distributions. CTAB-GAN is extensively evaluated with the state of the art GANs that generate synthetic tables, in terms of data similarity and analysis utility. The results on five datasets show that the synthetic data of CTAB-GAN remarkably resembles the real data for all three types of variables and results in higher accuracy for five machine learning algorithms, by up to 17%. Additionally, to ensure greater security for training tabular GANs against malicious privacy attacks, differential privacy (DP) is studied and used to train CTAB-GAN with strict privacy guarantees. DP-CTAB-GAN is rigorously evaluated using state-of-the-art DP-tabular GANs in terms of data utility and privacy robustness against membership and attribute inference attacks. Our results on three datasets indicate that strict theoretical differential privacy guarantees come only after severely affecting data utility. However, it is shown empirically that these guarantees help provide a stronger defence against privacy attacks. Overall, it is found that DP-CTABGAN is capable of being robust to privacy attacks while maintaining the highest data utility as compared to prior work, by up to 18% in terms of the average precision score.

==> glossary.tex <==
% \addcontentsline{toc}{chapter}{Glossary}
\newglossaryentry{bohb}
{
    name=BOHB,
    description={Acronym of Bayesian Optimization and Hyperband, a state of the art HPO algorithm \cite{bohb}}
}

\newglossaryentry{bo}
{
    name=BO,
    description={Acronym of Bayesian Optimization, a class of search algorithms which are extensively used in black-box optimization processes}
}


\newglossaryentry{sh}
{
    name=SH,
    description={Successive Halving, a multi-armed bandit based HPO algorithm}
}


\newglossaryentry{hyperband}
{
    name=Hyperband,
    description={Hyperband, a multi-armed bandit based HPO algorithm \cite{hyperband}}
}

\newglossaryentry{rung}
{
    name=Rung,
    description={When describing Successive Halving, a rung refers to a batch of configurations that are to be evaluated for a fixed budget. Each termination cycle can also be referred to as a rung}
}


\newglossaryentry{bracket}
{
    name=Bracket,
    description={When describing Hyperband or BOHB, a bracket refers to an instance of a successive halving run}
}

\newglossaryentry{budget}
{
    name=Budget,
    text=budget,
    description={Budget refers to the means through which fidelities are defined in each of the multi-fidelity algorithms discussed in this thesis}
}


\newglossaryentry{budget_type}
{
    name=Budget type,
    text=budget type,
    description={Also called fidelity type, the budget type refers to the types of resource used in defining fidelities. In our thesis, we have considered epoch based budget, training dataset based budget and training duration based budget}
}

\newglossaryentry{budget_constraint}
{
    name=Budget constraints,
    text=budget constraint,
    description={Used in context of Hyperband and BOHB, budget constraints are frameworks used to define fidelities. For vanilla BOHB, specifying budget constraints involve setting the minimum budget, the maximum budget and the reduction parameter $\eta$. These terms have been studied further in chapter \ref{ch3}}
}

\newglossaryentry{epoch-budget}
{
    name=Epoch based budget,
    text=epoch based budget,
    description={In using epochs to define fidelities, we control the number of iterations for which the specified amount of training data samples are iterated through the model for learning the model parameters}
}

\newglossaryentry{trainset-budget}
{
    name=Trainset based budget,
    text=trainset based budget,
    description={In using proportions of training dataset to define fidelities, we control percentage of training data samples used in the training phase, as well as the number of iterations for which the specified amount of training data samples are iterated through the model for learning the model parameters}
}

\newglossaryentry{time-budget}
{
    name=Time based budget,
    text=time based budget,
    description={In using training duration to define fidelities, we control the amount of time spent on training the model, using the specified percentage of training data samples}
}

% \newglossaryentry{budget}
% {
%     name=Budget,
%     description={Budget refers to the means through which fidelities are defined in each of the multi-fidelity algorithms discussed in this thesis. }
% }

